CAPoW: Context-Aware AI-Assisted Proof of Work based DDoS Defense

Critical servers can be secured against distributed denial of service (DDoS) attacks using proof of work (PoW) systems assisted by an Artificial Intelligence (AI) that learns contextual network request patterns. In this work, we introduce CAPoW, a context-aware anti-DDoS framework that injects latency adaptively during communication by utilizing context-aware PoW puzzles. In CAPoW, a security professional can define relevant request context attributes which can be learned by the AI system. These contextual attributes can include information about the user request, such as IP address, time, flow-level information, etc., and are utilized to generate a contextual score for incoming requests that influence the hardness of a PoW puzzle. These puzzles need to be solved by a user before the server begins to process their request. Solving puzzles slow down the volume of incoming adversarial requests. Additionally, the framework compels the adversary to incur a cost per request, hence making it expensive for an adversary to prolong a DDoS attack. We include the theoretical foundations of the CAPoW framework along with a description of its implementation and evaluation.

==> DSN-tool-comments.tex <==
Review #15A
===========================================================================

Reviewer expertise
------------------
2. Some familiarity

Paper summary
-------------
The authors describe a software tool that aims at preventing DoS attacks on critucal servers by (1) using machine learning to detect abnormal behavior, and (2) when abnormal behavior is detected, requesting the clients solve puzzles of increasing difficulty, with the goal that misbehaving clients have their latency increased between requests.

Reasons to Accept
-----------------
- the paper addresses an important topic
- the paper is clearly written and presented
- the source code of the tool is available on Github

Reasons to Reject
-----------------
- the proposal does not seem to prevent very basic DoS attacks (see below)

Comments for authors
--------------------
I may have missed something reading the paper, but it seems to me that:

- the defense is based on the fact that the malicious clients will solve the puzzles they are sent. What is their incentive for doing so ? Simply senting requests in an abnormal manner will generate new puzzles at the server of increasing difficulty. Then, not solving the puzzles and sending bogus responses will make the server check those responses. So, the server sends puzzles, checks responses, and the latency of the malicious client is not increased. With many such clients, the DoS still occurs.

- the ability for a malicious agents to spoof the IP address of a genuine client permits to make the server think this genuine client is suspicious, yielding sending increasingly difficult puzzles to the genuine client, inducing a drop in latency (and a high consumption of resources) for genuine clients. So, even a single maicious client can general a high latency for all genuine clients if their traffic can be observed (as is assumed in the paper).

Overall, the claim that the proposed tool is a solution to DoS is an overstatement.

Can this paper become acceptable after a revision?
--------------------------------------------------
3. Yes, a revision can make the paper acceptable assuming the issues are
   addressed in the revision timeframe (2 weeks)

What should the authors improve in the revised version?
-------------------------------------------------------
- explain why a malicious client has to solve the puzzle
- explain why a malicious client cannot increase the latency of genuine clients


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #15B
===========================================================================

Reviewer expertise
------------------
3. Knowledgeable

Paper summary
-------------
This paper presents an AI-based defensive solution against DDOS attacks   that is based on the modeling of normal activity using ML models and the execution of proof of work puzzles that are adaptively tuned depending on whether the incoming requests are detected as benign or malicious. Context information are used to build ML models and to evaluate scoring functions to support anomaly detection. If the incoming request is detected as normal easy puzzles are sent to the users to be solved, while more difficult puzzles are generated for malicious requests which leads to a higher latency in processing those requests. The paper describes the main principles behind the design of this solution and presents an instance of the implementation of its core components. An evaluation is also performed using an example derived from the CIC-IDS2017 simulated dataset

Reasons to Accept
-----------------
- The paper presents a solution for addressing DDOS attacks with some interesting ideas to adaptively adpat to malicious requests

- The basic  principles behind the proposed solution are clearly described

- an implementation will be made publicly available on Github

Reasons to Reject
-----------------
- The paper is more focussed on the description of the design principles behind the proposed solution than on the implementation details as expected for a tool description paper, for instance about ML models and algorithms that have implemented  in the tool, the software technologies used to develop and integrate the different components, etc. 

- the tool has a narrow scope and may not be interesting to a large audience. Or at least this issue deserves to be discussed in the paper

- The paper lacks a discussion about the scalability and performance of the tool, the possibility to extend or reuse some of its components for other types applications, etc.

- The efficiency of the tool for defending against DDOS attack is not experimentally validated based on significant evaluation case

Comments for authors
--------------------
This paper addresses a relevant topic  that  fits the scope of the conference. The AI-based defensive solution against DDOS attacks that is based on the  adaptive execution of proof of work puzzles that are tuned depending on whether the incoming requests are detected as benign or malicious,  brings some interesting ideas to increase the latency of the requests that are detected as malicious, though one question that can be raised why not simply block the corresponding requests. 

The following concerns can also be raised and need to be addressed :

- The paper is more focussed on the description of the design principles behind the proposed solution than on the implementation details as expected for a tool description paper, for instance about ML models and algorithms that have implemented  in the tool, the software technologies used to develop and integrate the different components, etc. 

- the tool has a narrow scope and may not be interesting to a large audience. 

- The paper lacks a discussion about the scalability and performance of the tool,  as well as about the possibility to extend or reuse some of its components for other types applications, etc.

- The efficiency of the tool for defending against DDOS attack is not experimentally validated based on a significant  evaluation case.  The example presented in thge paper is rather simple and does provide convincing evidence about the practical relvance of the solution

Can this paper become acceptable after a revision?
--------------------------------------------------
4. No, there are too many issues to address in the revision timeframe


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #15C
===========================================================================

Reviewer expertise
------------------
2. Some familiarity

Paper summary
-------------
This tool paper presents CAPoW, a Proof of Work based DDoS defense "tool". The idea of the paper is that the tool learns normal behavior and if a user deviates from the normal behavior, different amount of work is imposed to the misbehaving user to slow down their attack. The tool assigns work adaptively and policies can be provided to control the PoW.

Reasons to Accept
-----------------
- The paper presents an interesting idea (but the practicality is questionable)
- The paper is well-written and would be relevant for DSN.

Reasons to Reject
-----------------
- It seems to me that the tool does not prevent a lot of common DDoD attacks (e.g., SYN flood, ICMP flood) - it only seems to work if the attacker agrees to execute the protocol
- This is a tool paper but the paper does not show how the tool would work in practice, that is, it seems the client end of the "tool" has not been implemented and the tool is only evaluated using a simulated data set.

Comments for authors
--------------------
There are many ways a web service protected by this tool can be attacked. For example, SYN flood or ICMP flood can overwhelm the server without even getting to the application level where the tool executes. An attacker can also send the initial request as often as they want and not even wait to receive the puzzle. The work that the web server has to do extract context and construct puzzle just adds more work to the server but has no impact on the attacker resource usage (since they just ignore the puzzle). Similarly since the adversary can spoof IP address, they can send requests from arbitrary number of fake IP addresses. 

For a tool paper, I would expect end-to-end implementation (including the user end point) and demonstration that this works in practice.

Can this paper become acceptable after a revision?
--------------------------------------------------
4. No, there are too many issues to address in the revision timeframe

What should the authors improve in the revised version?
-------------------------------------------------------
The authors should think how to make this idea work in practice.
